Approximate Hypergraph Vertex Cover and generalized Tuza's conjecture

A famous conjecture of Tuza states that the minimum number of edges needed to cover all the triangles in a graph is at most twice the maximum number of edge-disjoint triangles. This conjecture was couched in a broader setting by Aharoni and Zerbib who proposed a hypergraph version of this conjecture, and also studied its implied fractional versions. We establish the fractional version of the Aharoni-Zerbib conjecture up to lower order terms. Specifically, we give a factor $t/2+ O(\sqrt{t \log t})$ approximation based on LP rounding for an algorithmic version of the hypergraph Tur\'{a}n problem (AHTP). The objective in AHTP is to pick the smallest collection of $(t-1)$-sized subsets of vertices of an input $t$-uniform hypergraph such that every hyperedge contains one of these subsets. Aharoni and Zerbib also posed whether Tuza's conjecture and its hypergraph versions could follow from non-trivial duality gaps between vertex covers and matchings on hypergraphs that exclude certain sub-hypergraphs, for instance, a "tent" structure that cannot occur in the incidence of triangles and edges. We give a strong negative answer to this question, by exhibiting tent-free hypergraphs, and indeed $\mathcal{F}$-free hypergraphs for any finite family $\mathcal{F}$ of excluded sub-hypergraphs, whose vertex covers must include almost all the vertices. The algorithmic questions arising in the above study can be phrased as instances of vertex cover on simple hypergraphs, whose hyperedges can pairwise share at most one vertex. We prove that the trivial factor $t$ approximation for vertex cover is hard to improve for simple $t$-uniform hypergraphs. However, for set cover on simple $n$-vertex hypergraphs, the greedy algorithm achieves a factor $(\ln n)/2$, better than the optimal $\ln n$ factor for general hypergraphs.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we proved the fractional version of the generalized Tuza's conjecture by giving an approximation algorithm with a factor $\frac{t}{2}+o(t)$  for the algorithmic hypergraph Tur\'{a}n problem (\textsf{AHTP}).  
Our work also raises several natural directions to further explore: 
\begin{enumerate}
    \item Finding better algorithms and improved hardness results for \textsf{AHTP} is still wide open. Especially on the hardness front, the best hardness result (for any $t$) is the factor $2$ hardness of the vertex cover problem on graphs, under the Unique Games Conjecture. Towards this, an interesting open problem is to obtain $\omega(1)$ lowerbound on the integrality gap of the standard LP relaxation for \textsf{AHTP}.
    %But this could also be tricky given the fact that we do not understand the integral value of the LP relaxation on the complete $t$-uniform hypergraph instance~\cite{decain}.
    %\item $(t,k)$-version of $\textsf{AHTP}$: Throughout the paper, we have studied the problem of vertex cover on $H=G^{(t-1)}$ for a given $t$-uniform hypergraph $G$. An interesting generalization is the problem of vertex cover on $H=G^{(k)}$ for a $t$-uniform hypergraph $G$, for an arbitrary $1\leq k < t$. The case of $k=1$ is the standard vertex cover on $t$-uniform hypergraphs, and $k=t-1$ is the \textsf{AHTP}. Of special interest is the case when $k=2$: finding an $o(t^2)$ factor approximation algorithm or showing NP-hardness of finding one is an interesting open problem. 

\item The dual problem to \textsf{AHTP} is the maximum matching problem on $t$-blown-up hypergraphs. For the general case of the maximum matching problem on $t$-uniform hypergraphs, also known as $t$-set packing, Cygan~\cite{Cygan13} gave a local search algorithm that achieves an approximation factor of $\frac{t+1}{3}+\epsilon$ for any $\epsilon >0$. Can we get better algorithms for the maximum matching problem on $H=G^{(t-1)}$? On the hardness front, by a simple reduction from the independent set problem on graphs with maximum degree $t$\cite{AKS11,Chan16}, it follows that the maximum matching problem on $t$-uniform \emph{simple} hypergraphs is NP-hard to approximate better than $\Omega\left(\frac{t}{\log ^2t}\right)$.

\end{enumerate}
The hardness of the coverage version of \textsf{AHTP}, \textit{Johnson Coverage Hypothesis}(JCH)~\cite{CKL20} has various implications for fundamental clustering problems in Euclidean metrics. The coverage version of the set cover problem, known as Maximum coverage has $1-\frac{1}{e}+\epsilon$ hardness which can be proved by a simple reduction from the $\ln n$ hardness of set cover. Whether such progress towards JCH can be made assuming some form of hardness of \textsf{AHTP} is an interesting open problem.

